KRONC: Keypoint-based Robust Camera Optimization for 3D Car Reconstruction

The three-dimensional representation of objects or scenes starting from a set of images has been a widely discussed topic for years and has gained additional attention after the diffusion of NeRF-based approaches. However, an underestimated prerequisite is the knowledge of camera poses or, more specifically, the estimation of the extrinsic calibration parameters. Although excellent general-purpose Structure-from-Motion methods are available as a pre-processing step, their computational load is high and they require a lot of frames to guarantee sufficient overlapping among the views. This paper introduces KRONC, a novel approach aimed at inferring view poses by leveraging prior knowledge about the object to reconstruct and its representation through semantic keypoints. With a focus on vehicle scenes, KRONC is able to estimate the position of the views as a solution to a light optimization problem targeting the convergence of keypoints' back-projections to a singular point. To validate the method, a specific dataset of real-world car scenes has been collected. Experiments confirm KRONC's ability to generate excellent estimates of camera poses starting from very coarse initialization. Results are comparable with Structure-from-Motion methods with huge savings in computation. Code and data will be made publicly available.

==> tables/ablation_synt_noise.tex <==
\definecolor{myrowcolor}{HTML}{F5F5F5}

% \begin{table}[t]
%     \centering
%     \begin{tabular}{cc c|c cc | cc c}
%         \toprule
         
%         \textbf{$\omega$Rot. (°)} & \textbf{$\omega$Trans. (cm)} & & & Rot. (°)~$\downarrow$ & Trans. (cm)~$\downarrow$ & PSNR~$\uparrow$ & SSIM~$\uparrow$ & LPIPS~$\downarrow$   \\
%          \midrule
%          5 &  $0.7 \times 10^2$ &&& 0.75 & 3.07 & 34.34 & 0.982 & 0.014 \\
%          \rowcolor{myrowcolor}
%          5 & $1.5 \times 10^2$ &&& 1.35 & 3.10 & 34.34 & 0.982 & 0.014 \\
%          6 &  $2 \times 10^2$ & && 3.79 & 3.16 & 34.26 & 0.982 & 0.014 \\
%          \rowcolor{myrowcolor}
%          6 & $2.5 \times 10^2$ &&& 2.34 & 2.13 & 34.16 & 0.981 & 0.014 \\
%          7 &  $3 \times 10^2$ & && 6.54 & 6.21 & 33.66 & 0.979 & 0.017 \\

%          \bottomrule
%     \end{tabular}

%         \vspace{.25cm}
%     \caption{Ablation study on the different amount of noise on rotation and translation. Results are obtained with the GaussianSplatting~\cite{kerbl20233d} baseline and averaged over the CarPatch dataset.}
%     \label{tab:tab_ablation_synt_noise}
% \end{table}



% \begin{table}[t]
%     \centering
%     \begin{tabular}{c c|c c | cc c}
%         \toprule
         
%         (\textbf{$\omega$Rot. (°)}, \textbf{$\omega$Trans. (cm)}) & & & (Rot. (°)~$\downarrow$  Trans. (cm)~$\downarrow$) & PSNR~$\uparrow$ & SSIM~$\uparrow$ & LPIPS~$\downarrow$   \\
%          \midrule
%          (5 ,  $0.7 \times 10^2$) &&& (0.75,3.07) & 34.34 & 0.982 & 0.014 \\
%          \rowcolor{myrowcolor}
%          (5 , $1.5 \times 10^2$) &&& (1.35,3.10) & 34.34 & 0.982 & 0.014 \\
%          (6 , $2 \times 10^2$) & && (3.79,3.16) & 34.26 & 0.982 & 0.014 \\
%          \rowcolor{myrowcolor}
%          (6 , $2.5 \times 10^2$) &&& (2.34,2.13) & 34.16 & 0.981 & 0.014 \\
%          (7 , $3 \times 10^2$) & && (6.54,6.21) & 33.66 & 0.979 & 0.017 \\

%          \bottomrule
%     \end{tabular}

%         \vspace{.25cm}
%     \caption{Ablation study on the different amount of noise on rotation and translation. Results are obtained with the GaussianSplatting~\cite{kerbl20233d} baseline and averaged over the CarPatch dataset.}
%     \label{tab:tab_ablation_synt_noise}
% \end{table}

%

==> tables/ablation_synth_views.tex <==
\definecolor{myrowcolor}{HTML}{F5F5F5}

\begin{table}[t]
   \centering
   \resizebox{\linewidth}{!}{
   \begin{tabular}{c cccc}
       \toprule
        \textbf{\# Train poses} & \textbf{Poses} & PSNR~$\uparrow$ & SSIM~$\uparrow$ & LPIPS~$\downarrow$ \\
         \midrule
         80 & GT & 34.86 & 0.982
         & 0.014 \\
         \rowcolor{myrowcolor}

         60 & GT & 33.78 & 0.978
         & 0.017 \\
         40 & GT & 32.96 & 0.974 & 0.019 \\
        \midrule
         80 & Optimized & 31.36 & 0.973 & 0.019 \\
        \rowcolor{myrowcolor}
         60 & Optimized & 30.51 & 0.967
         & 0.022 \\
         40 & Optimized & 29.79 & 0.963 & 0.025 \\
        \bottomrule
   \end{tabular}
   }
   \caption{Ablation study on the different number of training camera poses. Results are obtained with the GaussianSplatting~\cite{kerbl20233d} baseline and averaged on the CarPatch dataset.}
   \label{tab:tab_ablation_synt_views}
\end{table}

==> tables/results_real_old.tex <==
\definecolor{myrowcolor}{HTML}{F5F5F5}

\begin{table*}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ll cc ccc ccc}
        \toprule
        & & & & \multicolumn{3}{c}{\textbf{Full scene}} & \multicolumn{3}{c}{\textbf{Masked vehicle}} \\
        [0.35em]
         \textbf{Env} & \textbf{Vehicle} & \textbf{Init Pose} & \textbf{\# Optim. Cameras} & PSNR~$\uparrow$ & SSIM~$\uparrow$ & LPIPS~$\downarrow$ & PSNR~$\uparrow$ & SSIM~$\uparrow$ & LPIPS~$\downarrow$ \\
         \midrule
         Env1 & Ford-Focus & COLMAP & - & 29.11 & 0.916 & 0.089 & 28.37 & 0.959 & 0.036 \\
         \rowcolor{myrowcolor}
         Env1 & Fiat-500L & COLMAP & - & 26.94 & 0.892 & 0.115 & 25.12 & 0.930 & 0.061 \\
         Env1 & Hyundai-i10 & COLMAP & - & 29.38 & 0.918 & 0.097 & 29.45 & 0.971 & 0.026 \\
         \rowcolor{myrowcolor}
         Env2 & Fiat-500L & COLMAP & - & 28.15 & 0.922 & 0.117 & 28.60 & 0.945 & 0.048 \\
         Env2 & Toyota-Yaris & COLMAP & - & 28.90 & 0.936 & 0.115 & 29.18 & 0.957 & 0.029 \\
         \rowcolor{myrowcolor}
         Env3 & Toyota-Yaris & COLMAP & - & 31.00 & 0.948 & 0.065 & 33.31 & 0.983 & 0.017 \\
         Env3 & Hyundai-i10 & COLMAP & - & 30.95 & 0.942 & 0.072 & 31.11 & 0.974 & 0.025 \\
         \midrule
          Env1 & Ford-Focus & Trajectory & 161/161
          & 21,97 & 0.696 & 0.296 & 23,41 & 0,888 & 0.081 \\
         \rowcolor{myrowcolor}
         Env1 & Fiat-500L & Trajectory & 124/143 
         & 20.52 & 0.652 & 0.318 & 21.56 & 0.835 & 0.121 \\
         Env1 & Hyundai-i10 & Trajectory & 121/123 
         & 21,46 & 0.666 & 0.296 & 23.38 & 0.896 & 0.070 \\
         \rowcolor{myrowcolor}
         Env2 & Fiat-500L & Trajectory & 67/94  
         & 16.94 & 0.660 & 0.359 & 19.20 & 0.769 & 0.176 \\
         Env2 & Toyota-Yaris & Trajectory & 90/91 
         & 17.68 & 0.727 & 0.348 & 21.54 & 0.836 & 0.125 \\
         \rowcolor{myrowcolor}
        Env3 & Toyota-Yaris & Trajectory & 116/116
         & 19.06 & 0,601 & 0.396 & 21.23 & 0.850 & 0.130 \\
        Env3 & Hyundai-i10 & Trajectory & 107/123
         & 18.27 & 0.582 & 0.405 & 22.88 & 0.892 & 0.091 \\
         \bottomrule
    \end{tabular}
    }
    \vspace{.25cm}
    \caption{Quantitative results on the KRONC dataset. The GaussianSplatting~\cite{kerbl20233d} baseline trained with COLMAP poses and an optimized standard trajectory.}
    \label{tab:tab_results_real}
\end{table*}

==> tables/results_real_traj_vs_opt.tex <==
\definecolor{myrowcolor}{HTML}{F5F5F5}

\begin{table*}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ll c ccc ccc}
        \toprule
        & & & \multicolumn{3}{c}{\textbf{Full scene}} & \multicolumn{3}{c}{\textbf{Masked vehicle}} \\
        [0.35em]
         \textbf{Env} & \textbf{Vehicle} & \textbf{Trajectory} & PSNR~$\uparrow$ & SSIM~$\uparrow$ & LPIPS~$\downarrow$ & PSNR~$\uparrow$ & SSIM~$\uparrow$ & LPIPS~$\downarrow$ \\
         \midrule
         Env1 & Ford-Focus & Coarse & 18.15 & 0.520 & 0.507 & 15.85 & 0.720 & 0.277 \\
         \rowcolor{myrowcolor}
         Env1 & Fiat-500L & Coarse & 16.38 & 0.472 & 0.533 & 13.97 & 0.658 & 0.336 \\
         Env1 & Hyundai-i10 & Coarse & 15.01 & 0.435 & 0.537 & 14.88 & 0.722 & 0.271 \\
         \rowcolor{myrowcolor}
         Env2 & Fiat-500L & Coarse & 14.77 & 0.582 & 0.465 & 17.25 & 0.719 & 0.257 \\
         Env2 & Toyota-Yaris & Coarse & 15.52 & 0.637 & 0.467 & 16.75 & 0.748 & 0.244 \\
         \midrule
         Env1 & Ford-Focus & Optimized & 20.31 & 0.633 & 0.364 & 21.49 & 0.851 & 0.115 \\
         \rowcolor{myrowcolor}
         Env1 & Fiat-500L & Optimized & 17.36 & 0.556 & 0.435 & 18.38 & 0.768 & 0.193 \\
         Env1 & Hyundai-i10 & Optimized & 17.79 & 0.568 & 0.393 & 21.14 & 0.863 & 0.103 \\
         \rowcolor{myrowcolor}
         Env2 & Fiat-500L & Optimized & 12.68 & 0.573 & 0.492 & 15.35 & 0.710 & 0.261 \\
         Env2 & Toyota-Yaris & Optimized & 15.53 & 0.662 & 0.426 & 18.80 & 0.793 & 0.172 \\
         \bottomrule
    \end{tabular}
    }
    \caption{Quantitative results on the KRONC dataset. We use the GaussianSplatting~\cite{kerbl20233d} baseline comparing the results using the coarse and optimized trajectory.}
    \label{tab:tab_results_real_traj_vs_opt}
\end{table*}

==> tables/results_synthetic_noisy_vs_opt.tex <==
\definecolor{myrowcolor}{HTML}{F5F5F5}
\definecolor{first}{HTML}{dec546}
\definecolor{second}{HTML}{d7d7d7}
\definecolor{third}{HTML}{7e4205}

\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcc ccc r}
        \toprule
         \textbf{Dataset} & \textbf{Poses} & PSNR~$\uparrow$ & SSIM~$\uparrow$ & LPIPS~$\downarrow$ \\
         \midrule
         \textsc{Bmw} & Noisy & 14.24 & 0.864 & 0.149 \\
         \rowcolor{myrowcolor}
         \textsc{Tesla} & Noisy & 14.38 & 0.851 & 0.161 \\
         \textsc{Smart} & Noisy & 14.04 & 0.896 & 0.113 \\
         \rowcolor{myrowcolor}
         \textsc{Mbz$_1$} & Noisy & 14.01 & 0.857 & 0.143 \\
         \textsc{Mbz$_2$} & Noisy & 13.82 & 0.849 & 0.148 \\
         \rowcolor{myrowcolor}
         \textsc{Ford} & Noisy & 11.19 & 0.758 & 0.261 \\
         \textsc{Jeep} & Noisy & 13.27 & 0.831 & 0.172 \\
         \rowcolor{myrowcolor}
         \textsc{Volvo} & Noisy & 13.57 & 0.855 & 0.153 \\
         \midrule
         \textsc{Bmw} & Optimized & 32.55 & 0.979 & 0.016 \\
         \rowcolor{myrowcolor}
         \textsc{Tesla} & Optimized & 33.35 & 0.981 & 0.015 \\
         \textsc{Smart} & Optimized & 33.35 & 0.982 & 0.012 \\
         \rowcolor{myrowcolor}
         \textsc{Mbz$_1$} & Optimized & 31.25 & 0.978 & 0.014 \\
         \textsc{Mbz$_2$} & Optimized & 31.73 & 0.977 & 0.015 \\
         \rowcolor{myrowcolor}
         \textsc{Ford} & Optimized & 28.44 & 0.947 & 0.036 \\
         \textsc{Jeep} & Optimized & 29.80 & 0.970 & 0.020 \\
         \rowcolor{myrowcolor}
         \textsc{Volvo} & Optimized & 30.45 & 0.970 & 0.019 \\
         \bottomrule
    \end{tabular}
    }
    \caption{Quantitative results on each scene of the CarPatch dataset. We use the GaussianSplatting~\cite{kerbl20233d} baseline comparing the results using the poses before and after the KRONC optimization.}
    \label{tab:tab_synt_noisy_vs_opt_results}
\end{table}
